DualVector: Unsupervised Vector Font Synthesis with Dual-Part Representation

Automatic generation of fonts can be an important aid to typeface design. Many current approaches regard glyphs as pixelated images, which present artifacts when scaling and inevitable quality losses after vectorization. On the other hand, existing vector font synthesis methods either fail to represent the shape concisely or require vector supervision during training. To push the quality of vector font synthesis to the next level, we propose a novel dual-part representation for vector glyphs, where each glyph is modeled as a collection of closed "positive" and "negative" path pairs. The glyph contour is then obtained by boolean operations on these paths. We first learn such a representation only from glyph images and devise a subsequent contour refinement step to align the contour with an image representation to further enhance details. Our method, named DualVector, outperforms state-of-the-art methods in vector font synthesis both quantitatively and qualitatively. Our synthesized vector fonts can be easily converted to common digital font formats like TrueType Font for practical use. The code is released at https://github.com/thuliu-yt16/dualvector.

==> chapters/method.tex <==


\section{Method}
In this section, we first illustrate the proposed dual-part representation for vector fonts and then introduce \sysname for training this representation from glyph images and how the trained model can be used for font vectorization and generation. 


\subsection{Dual Part Representation}
In our work, we adopt a joint representation of image and vector for fonts, shown in \cref{fig:method}. In the latent space, which both the two modalities share, we associate each glyph with a latent code $z \in \mathbf{R}^d$ produced by the task-specific encoding process. The latent code $z$ is fed into two decoding branches to form a vector representation and an image representation respectively. The output of the vector branch is further processed by a contour refinement module and refined to generate the final contour representation, where the image representation provides guidance on the details. The three parts are described as follows. 

\subsubsection{Vector Branch}
This branch is responsible for producing a vector representation of the glyph given the latent code $z$. A typical approach is to process $z$ with a sequence decoding model (e.g. RNN, LSTM, Transformer) and predict the control points on the contours in time step order. The main limitation of such a method is the ambiguity of SVG commands, which requires a subsequent Mixture Density Network (MDN) to describe the distribution of the next predicted instance, which is revealed in \cite{deepvecfont, learned-svg}. The extra MDN will also bring the location shift issue. In addition, direct regression of SVG commands requires explicit supervision, which limits the generality of this method to objects other than fonts. 

In our dual part representation, we consider the parametric B\'ezier closed paths as our basic primitives. This is designed for several following reasons: firstly, B\'ezier paths are powerful enough to approximate various shapes; secondly, the boolean operations between them are closed in nature; thirdly, they are widely used in modern font design, making the synthesized results highly applicable.

For convenience, a triplet of control points $(\bm{a},\bm{b},\bm{c})$ below denotes a quadratic B\'ezier curve $B(\cdot; \bm{a}, \bm{b}, \bm{c})$ controlled by the three points $\bm{a},\bm{b},\bm{c}$:
\begin{equation}
    B(t;\bm{a},\bm{b},\bm{c}) = (1-t)^2\bm{a} + (1-t)t\bm{b}+t^2\bm{c}, t\in [0,1]
\end{equation}
For a given  $z$, the path decoder $\mathcal{D}_P$ consumes it and outputs $N$ closed solid B\'ezier paths $\{P_i\}_{i=1}^N$. 
\begin{equation}
    \{\bm{x}_{i, j}\} = \mathcal{D}_P(z), 1 \le i \le N, 1 \le j \le 2M
\end{equation}
Each path $P_i$ is defined by $M$ connected quadratic B\'ezier curves $\{B_{i,j}(\bm{x}_{i,2j-1}, \bm{x}_{i,2j}, \bm{x}_{i,2j+1})\}_{j=1}^M$ ($\bm{x}_{i, 2M+1} = \bm{x}_{i, 1}$). The occupancy field of a closed path $P_i$ is given as 
\begin{equation}
    \mathcal{O}_{P_i}(\bm{x}) = \left\{\begin{array}{cc}
       1  ,& \bm{x} \in P_i \\
       0  ,& \bm{x} \notin P_i
    \end{array}\right.
\end{equation}
The entire glyph shape $g$ is denoted as the union of $\{P_i\}_{i=1}^N$. We normalize the coordinate range of the glyph to $[-1,1]^2$. Thus given any point $\bm{x}$ on the canvas $[-1,1]^2$, we can calculate whether it is inside the represented glyph by a maximum operation, leading to the occupancy field of $g$:
\begin{equation}
    \mathcal{O}(\bm{x}) = \max_i \mathcal{O}_{P_i}(\bm{x}) = \left\{\begin{array}{cc}
       1  ,& \bm{x} \in \cup_i P_i \\
       0  ,& \bm{x} \notin \cup_i P_i
    \end{array}\right. 
\end{equation}

The above representation is easy to model fonts with many convex curves on the contour while struggling to reconstruct shapes with holes, e.g. B,O. Therefore, in practice, we assign to each path $P_i$ a negative path $Q_i$ paired with it, and we term this pair $(P_i, Q_i)$ as the ``dual part", which is the origin of our method name \sysname. $\mathcal{D}_P$ is responsible for predicting the positive paths $\{P_i\}_{i=1}^N$ and also the negative ones $\{Q_i\}_{i=1}^N$. 
$g$ is represented as $\cup_i (P_i - Q_i)$. The occupancy field $\mathcal{O}$ is then reformatted as:
\begin{equation}
    \mathcal{O}(\bm{x}) = \max_i [\min(\mathcal{O}_{P_i}(\bm{x}), 1-\mathcal{O}_{Q_i}(\bm{x}))] = \left\{\begin{array}{cc}
       1  ,& \bm{x} \in g \\
       0  ,& \bm{x} \notin g
    \end{array}\right. 
\end{equation}

Even though $\mathcal{O}$ is the analytical occupancy field of $g$, it is not differentiable w.r.t the parameters of paths. Therefore, in order to apply gradient descent, we calculate the approximate occupancy field $\hat{\mathcal{O}}$ from $g$'s signed distance field. Since the distance $d(p; B)$ from any point $p$ to the B\'ezier curve $B$ can be given analytically, the SDF of a path can be calculated differentiably w.r.t. its control points as follows,
\begin{equation}
    s_{P_i}(\bm{x}) = [2\mathcal{O}_{P_i}(\bm{x}) - 1]\min_j d(\bm{x};B_{i,j})
\end{equation}
Following the previous vector graphics rasterization works\cite{randomaccess,diffvg,multi-implicit}, we approximate $\mathcal{O}$ by analytical pixel pre-filtering with a parabolic kernel $\alpha$:

\begin{equation}
\begin{aligned}
    & \hat{\mathcal{O}}_{P_i}(\bm{x}) = \alpha(s_{P_i}(\bm{x}))\\
    & \hat{\mathcal{O}}= \max_i [\min(\hat{\mathcal{O}}_{P_i}, 1-\hat{\mathcal{O}}_{Q_i})] 
\end{aligned}
\end{equation}
$\hat{\mathcal{O}}$ is currently a differentiable occupancy field w.r.t path parameters and of course parameters of $\mathcal{D}_P$ and $\mathcal{E}$. 

\subsubsection{Image Branch}

This branch maps $z$ to a raster image $\mathcal{I}$ of the glyph it represents. Here we adopt a convolution-based decoder $\mathcal{D}_I$.   

\begin{equation}
    \mathcal{I} = \mathcal{D}_I(z)
\end{equation}
where the raster image $\mathcal{I}$ is a gray-scale image in shape $H\times W$. It could provide detailed shape guidance to further refine the global contour. 

\subsubsection{Contour Refinement Module}
Although the part-wise representation outputted by the vector branch can already be rendered vectorially, there still exists a gap between it and today's standard representation for shape. Therefore, in this module, we first convert the part-wise representation into the contour of the glyph $\partial \mathcal{O}$ with the off-the-shelf tool Paper.js\cite{paperjs}. It can perform arbitrary boolean operations on SVG paths. 
Here the contour $\partial \mathcal{O}$ is a set of K closed B\'ezier paths.
\begin{equation}
    \partial \mathcal{O} = \{C_1, C_2, ..., C_K\} 
\end{equation}
where $K$ denotes the number of independent paths. Each individual part or hole increases $K$ by 1. $C_i$ is currently a closed B\'ezier paths composed of $l_i$ quadratic B\'ezier segments $\{\hat{B}_{i,j}(\bm{\hat{x}}_{i,2j-1}, \bm{\hat{x}}_{i,2j}, \bm{\hat{x}}_{i,2j+1})\}_{j=1}^{l_i}$. %The number of segments per path $l_i$ is variable and is determined by the actual calculations. 

% To obtain the contour $\partial \mathcal{O}$ from the part-wise representation, we can iterate through all the pair $(P_i, Q_i)$. Let $\mathcal{O}$ with subscript $k$ be the occupancy field of the union of first $k$ path pairs $\cup_{i=1}^k (P_k - Q_k)$. 
% At the $k$-th iteration step, we first compute the contour of $P_k - Q_k$ by intersecting their B\'ezier curve segments. To be concrete, we intersect all B\'ezier segments of $P_k$ and $Q_k$ separately and split those B\'ezier segments that are crossed at the intersection.  points. There is a natural observation that for any B\'ezier segment on $\partial(P_k - Q_k)$, it is either a segment that already exists in $P_k$ or $Q_k$ or a sub-curve of that segment. So, after the segment splitting, we have independent B\'ezier curves that do not intersect each other, each of which either completely lies in the interior of $P_k - Q_k$ or on $\partial(P_k - Q_k)$. We then remove those curves that are in the interior by testing $\mathcal{O}_{P_k - Q_k}(\bm{x})$ for any point $x$ on the curve and connect the remaining ones in order to obtain $\partial(P_k - Q_k)$. After the above calculation, we have actually completed a subtract boolean operation for the boundary of two paths. The process we get the contour of $\mathcal{O}_{k}$ from those of $\mathcal{O}_{k-1}$ and $P_k - Q_k$ is similar. One difference is that we need to perform a path-wise union operation for $P_k - Q_k$ and each individual piece of $\partial \mathcal{O}_{k-1}$ and aggregate the results. The other is that we test $\mathcal{O}_k(\bm{x})$ when removing interior segments.  

After conversion to the contour representation, we exploit the image output to further refine $\partial \mathcal{O}$ with  differentiable rendering techniques (e.g. DiffVG\cite{diffvg}). $\mathcal{I}$ could naturally serve as a raster version of the occupancy field $\mathcal{O}$. During the refinement, we devise several refining strategies to improve the quality and efficiency of the representation:

\paragraph{Simplification}
%We substitute a group of control points with their average value if all of them are close enough. 
To improve the efficiency of the contour representation, we replace those B\'ezier curve segments with a straight line segment connecting its endpoints if they are close enough. For a B\'ezier segment $(\bm{a}, \bm{b}, \bm{c})$, we can simply tell how faithfully the segment $\bm{ac}$ could represent it by the angle between $\vec{\bm{ba}}$ and $\vec{\bm{bc}}$. Also, we examine if there exist two adjacent B\'ezier segments that could be replaced by a single one. Since all quadratic B\'ezier curves are parts of a parabola, we derive the parameters of the corresponding parabolas from control points and merge the two curves if these parameters are close. 
%All of these simplifying operations could be applied to both pre-refinement or post-refinement procedure.

\paragraph{Pruning}
Prior to refinement, some B\'ezier paths of the contour may enclose tiny or extremely thin regions which will confuse the contour refinement process and produce useless curves that converge near a point. We trim those closed paths $C_i$ with a tiny inner area.

\paragraph{Subdivision}
To improve the flexibility of the refinement process, we split long B\'ezier segments at their midpoints. 



% that satisfies $S(C_i) < S_T$ where $S(\cdot)$ denotes the area and $S_T$ is a fixed threshold.


 

\subsection{Implementation and Training Method}

In this subsection, we will dive into how we use the proposed representation in both the font reconstruction and generation tasks and list all the optimization targets and strategies we used for training and refinement. 

\subsubsection{Optimization Objectives}
Optimization objectives can be divided into those at training time and those at inference time. The training-time objectives are task-related. 

\paragraph{Font reconstruction}
The input to our system is a gray-scale image of a glyph and the output is the corresponding vector representation, which could also be  referred to as vectorization. The pixel image $\mathcal{I}_{g}$ of the glyph $g$ is first passed through an image encoder $\mathcal{E}$ to obtain the latent variable $z$. 
\begin{equation}
    z = \mathcal{E}(\mathcal{I}_g)
\end{equation}

It is then decoded by our representation into the raster output $\mathcal{I}$ and vector parts $\{(P_i, Q_i)\}_{i=1}^N$. We train the three components, $\mathcal{E}$, $\mathcal{D}_I$ and $\mathcal{D}_P$, simultaneously with the following loss function. 
\begin{equation}
    \mathcal{L} = \lambda_P\mathcal{L}_P + \lambda_I\mathcal{L}_I
    \label{loss:rec}
\end{equation}
where  
\begin{equation}
\begin{aligned}
\mathcal{L}_P & = \mathbb{E}_{\bm{x}\sim[-1,1]^2}[||\hat{\mathcal{O}}(\bm{x}) - \mathcal{I}_g(\bm{x})||_1] \\
\mathcal{L}_I & = ||\mathcal{I} - \mathcal{I}_g||_2 + \text{LPIPS}(\mathcal{I}, \mathcal{I}_g)
\end{aligned}
\end{equation}
Here \text{LPIPS}\cite{lpips} is the perceptual loss on images and $\lambda$'s balance different losses. 

\paragraph{Font generation}
The input is several style reference images $\{R_i\}_{i=1}^{N_R}$ along with the target character $T$. The number of references $N_R$ is variable in training so the model could accept a variable number of references during inference. The style references are first mapped to their features $\{f_i\}_{i=1}^{N_R}$ with an image encoder $\mathcal{E}_f$. 
We then apply stacked self-attention layers SA to aggregate these features to the style latent code $z_{style}$ with a variational head to enable brand-new font sampling. 
The target character first goes through a learnable character embedding layer and is then fused with $z_{style}$ to yield the latent code $z_T$ of the target glyph. The subsequent decoding process is the same as that for the reconstruction task. 
\begin{equation}
\begin{aligned}
    f_i & = \mathcal{E}_f(R_i) \\
    \mu, \sigma & = \text{SA}(f_1, f_2, ..., f_{N_R}) \\
    z_{style} & = \mu + \epsilon\sigma, \epsilon\sim\mathcal{N}(0,1) \\
    z_T & = \text{FFN}([z_{style}, T])
\end{aligned}
\end{equation}
To ease training, we first use the pre-trained $\mathcal{E}$ from the reconstruction task to encode ground truth output $g_T$ and train the encoding module with a latent variable guidance
\begin{equation}
    \mathcal{L}_{latent} = ||z_T - \mathcal{E}(g_T)||_2
\end{equation}
and a Kullback-Leibler divergence loss\cite{vae14}. 
\begin{equation}
    \mathcal{L}_{kl} = \text{KL}(\mathcal{N}(\mu, \sigma^2) || \mathcal{N}(0,1))
\end{equation}


In the next stage, the encoding module is fine-tuned along with the pre-trained $\mathcal{D}_I$ and $\mathcal{D}_P$ from the reconstruction task using the loss in \ref{loss:rec} with $\mathcal{L}_{kl}$. 

\vspace{-4mm}
\paragraph{Refinement}
Both the reconstruction and generation tasks share the same refinement process, that is, given $\partial{\mathcal{O}}$ and $\mathcal{I}$, produce the glyph contour in SVG format using inference-time optimization. 
% The vector branch output is first converted to the coarse glyph contour $\{C_i\}_{i=1}^K$. 
In optimization, we utilize DiffVG\cite{diffvg}, denoted as DR, to render the coarse contour in a differentiable manner. The control points of $\mathcal{O}$ is refined to minimize the following loss function
\begin{equation}
    \mathcal{L}_{refine} =  \mathcal{L}_{ras} + \lambda_{reg}\mathcal{L}_{reg} 
\end{equation}
where $\mathcal{L}_{render}$ is the photo-metric loss between the rasterized image and the image branch output. 
\begin{equation}
    % \mathcal{L}_{ras} =  ||\textit{DR}(\{C_i\}_{i=1}^K) - \mathcal{I}||_1
    \mathcal{L}_{ras} =  ||\text{DR}(\partial{\mathcal{O}}) - \mathcal{I}||_1
\end{equation}
The regularization term limits the overall length of $\mathcal{O}$. 
\begin{equation}
     \mathcal{L}_{reg} =  \sum_{i=1}^K \text{len}(C_i)
\end{equation}

\subsubsection{Warm-up with Unsigned Distance Fields}
% signed distance warmup 
Although the vector branch is end-to-end trainable, the gradient is sufficient only near the edges. Therefore, to solve gradient vanishing in most areas, we add an extra loss on the unsigned distance field of the vector parts to warm up the system. 

In general, for two closed curves $c_1, c_2$, not necessarily the closed B\'ezier paths we are talking about here, we cannot obtain their boolean operation result's SDF exactly by point-wise operations on their respective SDFs. In fact, we have 
\begin{equation}
    s_{c_1 \cup c_2}(\bm{x}) \left\{\begin{array}{cc}
       = \min (s_{c_1}(\bm{x}), s_{c_2}(\bm{x})) ,& \bm{x} \notin c_1 \cup c_2 \\
        \le \min (s_{c_1}(\bm{x}), s_{c_2}(\bm{x})) ,& \bm{x} \in c_1 \cup c_2
    \end{array}\right.
\end{equation}
for the union of two SDFs. The $\min(\cdot)$ operation gives a correct SDF outside but an incorrect interior SDF. Similarly, the $\max(\cdot)$ gives a correct interior SDF and an incorrect one outside for intersection. Therefore, it is hard to calculate the accurate SDF of the global glyph $s_{\mathcal{O}}$. Fortunately, our aim is to make the optimization go well early in the training, and we find that using an approximate unsigned distance field works too. Here we define the UDF $u$ as 
\begin{equation}
    u(\bm{x}) = \max(0, s(\bm{x}))
\end{equation}
in which case $\min(\cdot)$ will give a correct global field when we union two parts. The approximate unsigned distance field of the glyph $\hat{u}_g$ is computed as 
\begin{equation}
    \hat{u}_g = \min_i [\max(u_{P_i}, u_{Q_i})]
\end{equation}
where 
\begin{equation}
\begin{aligned}
    u_{P_i}(\bm{x}) & = \max(s_{P_i}(\bm{x}), 0) \\
    u_{Q_i}(\bm{x}) & = \max(-s_{Q_i}(\bm{x}), 0) 
\end{aligned}
\end{equation}
Thus, for the font reconstruction task, in the first several epochs, we use the following objectives to warm up training
\begin{equation}
\begin{aligned}
    \mathcal{L} & = \lambda_P\mathcal{L}_P + \lambda_I\mathcal{L}_I + \lambda_{u}\mathcal{L}_u\\
    \mathcal{L}_u & = \mathbb{E}_{\bm{x}\sim[-1,1]^2}[||\hat{u}_g(\bm{x}) - u_g(\bm{x})||_1]
\end{aligned}
\end{equation}
where the ground truth UDF $u_g$ is derived from the pixel image $g$. 

% \subsection{Part-Wise Representation}

% We represent a glyph as a union of $P$ solid basic parts, whose contours are closed B\'ezier paths. Each path consists of $N$ quadratic B\'ezier curves. 

% Our model is in an encoder-decoder architecture. We choose to represent each glyph as a latent vector $z$. The encoders have different designs depending on the tasks and are responsible to produce the latent vector. 
% The decoder part has two branches. One of them consumes $z$ and predicts the control points for basic parts. It is responsible to predict the coarse shape of the desired glyph. The other converts $z$ into the glyph image.

% But we find that the basic parts themselves could not faithfully reconstruct the glyph especially for the font generation task due to its limited representation power. So we devise another branch to recover the rasterized glyph image from $z$. The part and pixel representations are responsible for the construction of shape and local detail respectively. The basic parts could be further combined into the contour representation for fonts and refined with the pixel guidance using differentiable renderer. 



